Mean and variance estimation in high-dimensional heteroscedastic models with non-convex penalties

Despite its prevalence in statistical datasets, heteroscedasticity (non-constant sample variances) has been largely ignored in the high-dimensional statistics literature. Recently, studies have shown that the Lasso can accommodate heteroscedastic errors, with minor algorithmic modifications (Belloni et al., 2012; Gautier and Tsybakov, 2013). In this work, we study heteroscedastic regression with linear mean model and log-linear variances model with sparse high-dimensional parameters. In this work, we propose estimating variances in a post-Lasso fashion, which is followed by weighted-least squares mean estimation. These steps employ non-convex penalties as in Fan and Li (2001), which allows us to prove oracle properties for both post-Lasso variance and mean parameter estimates. We reinforce our theoretical findings with experiments.

==> data.tex <==
\section{Real Data Application}

Forecasting the gross domestic product (GDP) of a country based on
macroeconomic indicators is of significant interest to the economic
community.  We obtain both the country GDP figures (specifically we
use the GDP per capita using current prices in units of a `national
currency') and macroeconomic variables from the International Monetary
Fund's World Economic Outlook (WEO) database.  The WEO database
contains records for macroeconomic variables from 1980 to 2016 (with
forecasts).

To form our response variable, $\yb_{i,t}$, we form log-returns of the
GDP for each country ($i$) for each time point ($t$) after records
began and before the forecasting commenced (each country had a
different year at which forecasting began).  After removing missing
values, we obtained 31 variables that can be grouped into a few broad
categories: balance of payments, government finance and debt,
inflation, and demographics.  We apply various transformations,
including lagging and logarithms forming the vectors $\xb_{i,t}$.  We
fit the heteroscedastic AR(1) model with HIPPO.
\[
\yb_{i,t} = \xb_{i,t-1}' \betab + 
     \exp (\xb_{i,t-1}' \thetab) \epsilon_{i,t}
\]

In order to initially assess the heteroscedasticity of the data, we
form the LASSO estimator with the LARS package in R selecting with
BIC.  It is common practice when diagnosing heteroscedasticity to plot
the studentized residuals against the fitted values.  We bin the bulk
of the samples into three groups by fitted values, and observe the
box-plot of each bin by residuals (Figure \ref{fig:studres}).  It is
apparent that there is a difference of variances between these bins,
which is corroborated by performing a F-test of equal variances across
the second and third bins (p-value of $4\times10^{-6}$).  We further
observe differences of variance between country GDP log returns.  We
analyzed the distribution of responses separated by countries: Canada,
Finland, Greece and Italy.  The p-value from the F-test for equality
of variances between the countries Canada and Greece is $0.008$, which
is below even the pairwise Bonferroni correction of $0.0083$ at $0.05$
significance level.
This demonstrates heteroscedasticity in the WEO dataset, and we are justified in fitting non-constant variance.

We compare the results from HIPPO and HHR when applied to the WEO
data set.  The tuning parameters were selected with BIC over a grid for
$\lambda_S$ and $\lambda_T$.  The metrics used to compare the
algorithms are mean square error (MSE) defined by $\frac{1}{n} \sum_i
(y_{i,t} - \hat y_{i,t})^2$, the partial prediction score defined as
the average of the negative log likelihoods, and the number of
selected mean parameters and variance parameters.  We perform
$10$-fold cross validation to obtain unbiased estimates of these
metrics.  In Table \ref{tb:imf} we observe that HIPPO outperforms HHR
in terms of MSE and partial prediction score.

\begin{table}[t]
{
\hfill{}
\begin{tabular}{c@{\hspace{0.6cm}}cc}
& \underline{\acro} & \underline{HHR} \\ 
\vspace{-0.2cm}
\\
MSE         & 0.0089 & 0.0091 \\
$-\ell(\yb, \Xb; \hat\betab, \hat\thetab)$    & 0.4953 & 0.6783 \\
 $|\widehat S|$ & 5.4    & 8.9    \\
 $|\widehat T|$ & 8.2    & 5.1    \\
\hline
\hline
\end{tabular}
}
\hfill{}
\caption{
  Performance of \acro and HHR on WEO data averaged over 10 folds.
}
\label{tb:imf}
\end{table}




%%% Local Variables:
%%% TeX-master: "paper"
%%% End:




==> stage1.tex <==
\subsection{Stage 1 Proof}

\begin{theorem}
\label{thm:scad_stage1}
Define $S = \{j : \beta_j \neq 0\}$ and $\bar \sigma = \max_{i \in [n]} \sigma_i$.
Assume the following
\begin{equation}
  \tag{A1.1}
  \label{eq:A1_1}
  \bar \sigma \sqrt{\frac{\log p}{n}} = o(\lambda_m)  
\end{equation}
\begin{equation}
  \tag{A1.2}
  \label{eq:A1_2}
  \lambda_m = o(\min_{j \in S} \beta_j)  
\end{equation}
\begin{equation}
  \tag{A1.3}
  \label{eq:A1_3}
  \exists c > 0, \Lambda_{\min}(n^{-1}\Xb_S'\Xb_S) > c \textrm{ for n large enough}  
\end{equation}
\begin{equation}
  \tag{A1.4}
  \label{eq:A1_4}
  \max_{j \in [p]} \| \Xb_j \| = O(\sqrt{n \log p})  
\end{equation}
The vector $\hat\betab = (\hat\betab_S', \zero_{S^C}')'$, where
$\hat\betab_S = (\Xb_S'\Xb_S)^{-1}\Xb_S'\yb$, is a strict local
minimizer of \eqref{eq:stage1} for $n$ large enough.
\end{theorem}

\begin{proof}
From Theorem~1 in \cite{fan09nonconcave}, we need to show that $\hat
\betab$ satisfies
\begin{equation}
  \label{eq:proof:scad_mean:cond_1}
  \Xb_S'(\yb - \Xb\hat\betab) - n \sgn(\hat\betab_S)\odot
  \pen'_{\lambda}(\hat\betab_S) = \zero,
\end{equation}
\begin{equation}
  \label{eq:proof:scad_mean:cond_2}
  \norm{\Xb\uSc'(\yb - \Xb\hat\betab)}_\infty < n \pen'_\lambda(0+),
\end{equation}
and 
\begin{equation}
  \label{eq:proof:scad_mean:cond_3}
  \Lambda_{\min}(n^{-1}\Xb_S'\Xb_S) > \max_{j \in S}\ \{-\pen''_\lambda(|\hat\beta_j|)\},
\end{equation}
in order to show that $\hat\betab$ is a strict local minimizer.

Let $\Pcal_{\Xb_S}$ be the projection onto the column space of $\Xb_S$.
Then $\Xb \hat \betab = \Pcal_{\Xb_S} \yb$ because it is the OLS estimator and $\Xb_S'(\yb - \Xb\hat\betab) = \Xb_S' (\yb - \Pcal_{\Xb_S} \yb) = \zero$.  
Furthermore,
\[
\hat\betab_S - \betab_S = (\Xb_S'\Xb_S)^{-1}\Xb_S'\etab =
(\Xb_S'\Xb_S)^{-1}\Xb_S'\diag(e^{\Xb\thetab/2})\epsilonb.
\]
Define
\[
\Mb :=
(\Xb_S'\Xb_S)^{-1}\Xb_S'\diag(e^{\Xb\thetab})\Xb_S(\Xb_S'\Xb_S)^{-1}.
\]
Conditional on $\Xb$, using Lemma~\ref{lem:sum_sub_gaussian} we have
that $\eb_j'(\hat\betab_S - \betab_S)$ is subgaussian with parameter
$\sqrt{2M_{jj}}$, $j \in S$. 
Therefore 
\begin{equation}
  \label{eq:proof:scad_mean:1}
  \PP[\norm{\hat\betab_S - \betab_S}_\infty > t\ \big|\ \Xb]
  \leq 2s\exp\left( -\frac{t^2}{2\max_{j \in S} M_{jj}} \right).
\end{equation}
Define $\Ab_j = \Xb_S (\Xb_S'\Xb_S)^{-1}\eb_j$
\[
M_{jj} = \sum_k A_{jk}^2 \sigma_k^2 \le \bar \sigma^2 \| \Ab_j \|^2 = \bar \sigma^2 \eb_j (\Xb_S' \Xb_S)^{-1} \eb_j \le \frac{\bar \sigma^2}{nc}
\]
for $n$ large enough.
By assumption \eqref{eq:A1_1} we know that $\norm{\hat\betab_S - \betab_S}_\infty = o_\PP(\lambda)$, thus,
\begin{equation*}
\begin{aligned}
  \min_{j \in S} |\hat \beta_j| &
    \geq \min_{j \in S} |\beta_j| - \norm{\hat\betab_S -
      \betab_S}_\infty \\
    & \geq \beta_{\min} - \norm{\hat\betab_S - \betab_S}_\infty = \omega_\PP(\lambda)\\
\end{aligned}
\end{equation*}
by assumption \eqref{eq:A1_2}.
This gives us that $\pen'(\hat \betab_S) = \zero$ and $\max_{j
  \in S} \{-\pen_\lambda''(|\hat \beta_j|)\} = 0$ showing
\eqref{eq:proof:scad_mean:cond_1} and
\eqref{eq:proof:scad_mean:cond_3}.
\[
\Xb\uSc'(\yb - \Xb\hat\betab) = \Xb\uSc' (\Ib - \Pcal_{\xb_S}) \yb = \Xb\uSc' (\Ib - \Pcal_{\xb_S}) \diag(\sigmab) \epsilonb
\]
Hence, $\Xb_j'(\yb - \Xb\hat\betab)$ is subGaussian with parameter
\[
\|\Xb_j' (\Ib - \Pcal_{\xb_S}) \diag(\sigmab) \| \le \bar \sigma \|\Xb_j' (\Ib - \Pcal_{\xb_S})\| \le \bar \sigma \| \Xb_j \| \le \frac{n \lambda_m}{\sqrt{\log p}}
\]
by assumptions  \eqref{eq:A1_1} and  \eqref{eq:A1_4}.
This (after a judicious use of the union bound) completes \eqref{eq:proof:scad_mean:cond_2}.
\end{proof}


\begin{theorem}
If the assumption in Theorem \ref{thm:scad_stage1} are satisfied then
\[
\| \Xb (\betab - \hat \betab) \|^2 = O_\PP\left( \bar \sigma^2 s \right)
\]
\end{theorem}

\begin{proof}
Because $\hat \betab$ is the OLS estimator,
\[
\begin{aligned}
& \Xb (\betab - \hat \betab) = \Xb \betab - \Pcal_{\Xb_S} \yb = - \Pcal_{\Xb_S} (\sigmab \circ \epsilonb) \\
&\| \Xb (\betab - \hat \betab) \|^2 = \epsilonb' \diag(\sigmab) \Pcal_{\Xb_S} \diag(\sigmab) \epsilonb \\
&= O_\PP(\tr\left(\diag(\sigmab) \Pcal_{\Xb_S} \diag(\sigmab)\right)) \le \bar \sigma^2 \tr (\Pcal_{\Xb_S}) = \bar \sigma s
\end{aligned}
\]
by Lemma \ref{lem:chi_squared}.
\end{proof}




